PetFMM--A dynamically load-balancing parallel fast multipole library

Fast algorithms for the computation of $N$-body problems can be broadly classified into mesh-based interpolation methods, and hierarchical or multiresolution methods. To this last class belongs the well-known fast multipole method (FMM), which offers O(N) complexity. This paper presents an extensible parallel library for $N$-body interactions utilizing the FMM algorithm, built on the framework of PETSc. A prominent feature of this library is that it is designed to be extensible, with a view to unifying efforts involving many algorithms based on the same principles as the FMM and enabling easy development of scientific application codes. The paper also details an exhaustive model for the computation of tree-based $N$-body algorithms in parallel, including both work estimates and communications estimates. With this model, we are able to implement a method to provide automatic, a priori load balancing of the parallel execution, achieving optimal distribution of the computational work among processors and minimal inter-processor communications. Using a client application that performs the calculation of velocity induced by $N$ vortex particles, ample verification and testing of the library was performed. Strong scaling results are presented with close to a million particles in up to 64 processors, including both speedup and parallel efficiency. The library is currently able to achieve over 85% parallel efficiency for 64 processors. The software library is open source under the PETSc license; this guarantees the maximum impact to the scientific community and encourages peer-based collaboration for the extensions and applications.

==> conclusions.tex <==
%%   conclusions.tex
%%   input to CruzBarbaKnepleyJCP2008.tex


%\section{Conclusions}
%\label{conclusions}

    We have presented an extension of the Greengard-Gropp parallel complexity analysis for the \fmm which is suitable for
distributed computing. We thus consider partition quality in terms of both communication volume and load balance, absent
from the original analysis, in order to derive an optimally distributed algorithm. This algorithm can maintain good
performance with highly non-uniform particle distributions, heterogeneous computing environments, and low bandwidth
connections.

    We have also delivered an open source, extensible implementation of this algorithm, intended as a community
resource.  The software library is truly open source\footnote{According to the definition provided in \url{http://www.opensource.org/docs/definition.php}}, and distributed 
under the \petsc\ license, even less restrictive than the \textsc{bsd} license. This guarantees the maximum impact to the
scientific community and encourages peer-based collaboration for the extensions and applications.

Our original approach to parallelization relies on recasting the hierarchical space division represented by a tree structure, into a weighted graph generated from a model of the computational work and communications estimates. The optimal partitioning of the graph produces dynamical load balancing. Experiments showed that processor execution times were within 5\% of each other for 32 processors and within 7\% of each other for 64 processors, demonstrating the success of our load balancing strategy.
The parallelization strategy permitted almost complete reuse of the serial implementation, and due to its
simplicity, was effected with very little additional code. It has shown very good strong scaling on small clusters. 
The library is currently able to achieve over 90\% parallel efficiency for 32 processors, and over 85\% parallel efficiency for 64 processors. 
The largest problem size that has been run with the \PetFMM\ library at this point was 64 million particles in 64 processors.  

At present, we are working on exposing more concurrency in the algorithm to exploit multi-core architecture; our real goal here is to extend these results to large clusters, and also to heterogeneous systems, including programmable graphics processing units, \textsc{gpu}.  With respect to delivering scalability to larger numbers of processing, we are investigating a strategy based on recursive tree-cutting approach, where the methodology described here can generate large subtrees which are further cut to obtain sub-subtrees.

In terms of the extensibility of \PetFMM, the first and most straightforward extension is to introduce 3D capability.  Our methodology applies without modification to 3D, as our tree and particle objects are templated over the dimension. Moreover, the parallel model involving work and communications estimates, and the setup for optimization of the partition, all apply to 3D. The main modification here involves the implementation of a new kernel, incorporating the 3D series expansions, and tranlation/transformation operators.

Future extensions of \PetFMM include the implementation of different kernels, for example Lennard-Jones potential for molecular dynamics applications, and extensions to other transforms such as fast Gauss transform.  We expect more extensions can be provided in the future by peers who find \PetFMM to be a good starting point for their scientific applications. To encourage peer-based collaboration, we are working to deliver an official release by the end of the year,  consisting of a User's Manual, example code and verification methods.

==> intro.tex <==
%%   intro.tex
%%   input to CruzBarbaKnepleyJCP2008.tex

%\section{Introduction}
%\label{intro}


So-called $N$-body problems arise in many areas (\emph{e.g.} astrophysics, molecular dynamics, vortex methods, electrostatics). In these problems, the system is described by a set of $N$ particles, and the dynamics of the system is the result of the interactions that occur for every pair of particles. To calculate all such interactions, the total number of operations required normally scales as $N^2$.  
One useful way to mathematically express an $N$-body problem is by means of a matrix-vector multiplication, where the matrix is dense and represents the particle interactions, and the vector corresponds to the weights of the particles. Thus, the mat-vec product corresponds to the evaluation of all pairwise interactions. In a naive implementation, we would directly create the matrix in computer memory and then perform the multiplication with the vector. This naive approach would prove feasible only for small $N$, as the computational requirements in processing power and memory both grow as $N^2$. For this reason, many efforts have been directed at producing efficient implementations, capable of performing the mat-vec operation at reduced memory requirements and operation counts.  

The various methods for more efficient calculation of the particle interaction problem can be broadly classified in two types:  mesh-based interpolation methods, and hierarchical or multiresolution methods. The basic mesh-based method is the particle-mesh (\textsc{pm}) approach, in which particle information is interpolated onto a lattice, the field of interest is solved on the mesh by means of some grid-based method such as finite difference, and the field information is finally interpolated back to the particle locations \cite{HockneyEastman81}. (This method is also called particle-in-cell, \textsc{pic}.) In some applications, such as molecular dynamics, the smoothing at the short-range introduced by the interpolations in the \textsc{pm} method is unacceptable.  An alternative mesh-based method can then be used in which all near-field potentials are calculated directly, while far-field effects are calculated with the \textsc{pm} method; this is called the particle-particle/particle-mesh method (\textsc{p}$^3$\textsc{m}).

The second class of methods provides efficient computation of the interactions by means of a hierarchical or multilevel
approach. The main subset of this class performs a hierarchical subdivision of the computational domain, which is used to group particles at different length scales, and then
approximates the interactions of clusters of particles using series expansions.  The
approximation is applied to far-field interactions, while near-field interactions are summed directly. This type of
methods can be considered meshfree, and includes: tree codes~\cite{BarnesHut1986,Appel1985}, the fast multipole method (\fmm)~\cite{greengard+rokhlin1987}
and its variations~\cite{CarrierGreengardRokhlin88,Anderson92,YingBirosZorin2004,GimbutasRokhlin2003}. An alternative
multilevel method has been presented by Skeel~\cite{SkeelTezcanHardy02}, which instead of using series expansions for the far field approximations utilizes a multigrid approach. The approximation of the field is in this case performed after a splitting of the particle potentials into a smooth part (matching the far field) and a nonsmooth part (acting only in the near field).  While the nonsmooth (purely local) part can be calculated directly at low cost, a multigrid method is used to approximate the smooth component.  For this approximation, the method relies on gridded basis functions of compact support, like in \textsc{p}$^3$\textsc{m}, but unlike \textsc{p}$^3$\textsc{m} it provides acceleration via multiple grid levels, achieving \bigON\ complexity.  Thus, this method applies the multilevel approach via field decomposition, rather than spatial decomposition; it can perhaps be viewed as a hybrid of the mesh-based and hierarchical methods.  

In this paper, we present the theory and development of a parallel fast multipole library, \PetFMM\footnote{\PetFMM stands for `portable extensible toolkit for \fmm', as in \petsc, which is `portable extensible toolkit for scientific computing'.}, belonging to the \emph{meshfree} type of methods described above. The overarching goal is to unify the efforts in the development of \fmm-like methods into an open-source library, that provides a framework with the capacity to accommodate memory efficiency, parallelism and the data structures used for spatial decomposition. The software is implemented utilizing  \href{http://www.mcs.anl.gov/petsc/petsc-as/}{\petsc}, the parallel library for scientific computing developed over more than 17 years at Argonne National Laboratory~\cite{petsc-manual}.  At this point, we have a complete implementation of the \fmm in parallel, with dynamic load balancing provided by means of an optimization approach---minimizing inter-node communications and per-node computational work.  But a prominent feature of this implementation is that it is designed to be \emph{extensible}, so that it can effectively unify efforts involving many algorithms which are based on the same principles of the \fmm.  The perspectives for extensibility are described in this paper as well.

The development of this extensible parallel library for $N$-body interactions is important due to the programming difficulty associated with the \fmm algorithm, which has been a barrier for adoption and arguably diminished its potential impact. A critical stage in the maturation of a computational field begins with the widespread availability of community
software for the central algorithms. 
A good example is molecular dynamics, which blossomed after introduction of freely available packages, such as \textsc{charmm} \cite{CHARMM1983} and \textsc{namd} \cite{NAMD2005}.  Such game-changing community software does not exist for particle methods or for $N$-body computations in general.

The present paper does not merely describe a new parallel strategy and implementation, it also details an exhaustive model for the computation of tree-based $N$-body algorithms in parallel.  Our model is a significant extension of the time model developed in \cite{GreengardGropp1990}, which assumed a uniform distribution of the particles among processors and does not address load balancing or communication overheads.  With our  model, which includes both work estimates and communication estimates,  we are able to implement a method to provide a priori, automatic load balancing.

The first parallel implementations of the \fmm was that of Greengard and Gropp \cite{GreengardGropp1990}, on a shared memory computer.  They also presented a timing model for a perfectly balanced implementation, of which we say more in \S\ref{work}. More recent versions of the parallel \fmm have been presented in~\cite{Ying03anew,Have2003,Ogata2003,kurzakPettit2005}.  Many of these codes produce a partition of the data among processors based upon a
space-filling curve, as previously introduced for the case of parallel treecodes in~\cite{warren+salmon93}. Only
one of these parallel \fmm codes represents a supported, open source code available for community use. The \textsc{kifmm}3d code can be downloaded
and modified under the \textsc{gpl} license. It is not an implementation of the classic \fmm algorithm, however, but rather a
kernel-independent version developed by the authors. This algorithm does not utilize series expansions, but instead
uses values on a bounding surface of each subdomain obtained through an iterative solution method; these ideas are based on \cite{Anderson92}. The code does not appear to
allow easy extension to traditional \fmm, or to the other related algorithms alluded to above. Moreover, it does not
appear to be designed as an embedded library component, part of a larger multiphysics simulation.

This paper is organized as follows.  We present first a brief overview of the \fmm algorithm; this presentation is necessarily cursory, as a large body of literature has been written about this method.  A basic description, however, is necessary to agree on a common terminology for the rest of the paper. Our approach is to illustrate the method using graphical representations.  The following section (\S\ref{particle}) describes our client application code, the vortex particle method for simulation of incompressible flow at high Reynolds numbers.  In this method, the \fmm is one of two approaches commonly used to obtain the velocity of particles from the vorticity field information; the second approach (as in other $N$-body problems) is to interpolate information back and forth from a mesh, while solving for the field of interest on the mesh.  Although equally efficient---both can be \bigON---the extensive use of interpolations may introduce numerical diffusion, which is undesirable in certain applications. Next, \S\ref{parallel} discusses our parallelization strategy.  The goal is achieving optimal distribution of the computational work among processors and minimal communication requirement. Our approach to parallelization is original in the use of an optimization method to obtain the parallel partitioning. To be able to apply such an optimization, there is need for good estimates of the computational work required for algorithmic components, as well as communication requirements. The development of these estimates, in addition to memory estimates, is presented in \S\ref{work}.  The subsequent section (\S\ref{software}) presents details of our software design, implementation and verification carried out.  Results of computational experiments with the parallel software are presented in \S\ref{results}, and we end with some conclusions and remarks about future work.

Note that a very simple
and flexible, yet efficient and scalable code has been produced. The entire \PetFMM implementation of \fmm is only \oldstylenums{2600} lines of C$^{++}$,
including comments and blank lines. It is already freely downloadable from \url{http://petsc.cs.iit.edu/petsc/} and we welcome correspondence with potential users or those who wish to extend it for specific purposes.


